The decline of disruptive science and technology

Theories of scientific and technological change view discovery and invention as endogenous processes, wherein prior accumulated knowledge enables future progress by allowing researchers to, in Newton's words, "stand on the shoulders of giants". Recent decades have witnessed exponential growth in the volume of new scientific and technological knowledge, thereby creating conditions that should be ripe for major advances. Yet contrary to this view, studies suggest that progress is slowing in several major fields of science and technology. Here, we analyze these claims at scale across 6 decades, using data on 45 million papers and 3.5 million patents from 6 large-scale datasets. We find that papers and patents are increasingly less likely to break with the past in ways that push science and technology in new directions, a pattern that holds universally across fields. Subsequently, we link this decline in disruptiveness to a narrowing in the use of prior knowledge, allowing us to reconcile the patterns we observe with the "shoulders of giants" view. We find that the observed declines are unlikely to be driven by changes in the quality of published science, citation practices, or field-specific factors. Overall, our results suggest that slowing rates of disruption may reflect a fundamental shift in the nature of science and technology.

==> commands.tex <==

% blackboard bold for naturals, integers, etc.
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

%comments shown

\newcommand{\russ}[1]{\textcolor{orange}{(Russ says: {#1})}}
\newcommand{\mike}[1]{\textcolor{blue}{(Mike says: {#1})}}

\newcommand{\beginsupplement}{%
        \setcounter{table}{0}
        \renewcommand{\thetable}{S\arabic{table}}%
        \setcounter{figure}{0}
        \renewcommand{\thefigure}{S\arabic{figure}}%
     }


% text commands
\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbb}
\newcommand{\mf}{\mathfrak}
\newcommand{\tn}[1]{\textnormal{#1}}


% greek lower case
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\w}{\omega}
\newcommand{\s}{\sigma}
\newcommand{\ph}{\varphi}
\newcommand{\p}{\partial}
\renewcommand{\t}{\tau}
\renewcommand{\th}{\theta}
\newcommand{\z}{\zeta}

% greek upper case
\newcommand{\Om}{\Omega}
\newcommand{\Ga}{\Gamma}
\newcommand{\Si}{\Sigma}
\newcommand{\La}{\Lambda}

% script upper case
\newcommand{\A}{\mathscr{A}}
\newcommand{\B}{\mathscr{B}}


%% counter for labels in description env
\newcounter{desccount}
\newcommand{\descitem}[1]{%
  \item[#1] \refstepcounter{desccount}\label{#1}
}
\newcommand{\descref}[1]{\hyperref[#1]{#1}}


% pullback functions
\newcommand{\fst}{f^{*}}
\newcommand{\gst}{g^{*}}


% misc

\newcommand{\uniflim}{\operatorname{unif}\lim}
\newcommand{\unifr}{\xrightarrow{\operatorname{unif.}}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\hr}{\hookrightarrow}
\newcommand{\li}{\lambda_I}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lbar}{\left|}
\newcommand{\rbar}{\right|}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}

\newcommand\mattwo[4]{\left(\begin{smallmatrix}
			{#1} & {#2}\\
     			{#3} & {#4}
                     \end{smallmatrix}\right)}
\newcommand\mattres[9]{\left(\begin{smallmatrix}
			{#1} & {#2}&{#3}\\
     			{#4} & {#5}&{#6}\\
     				{#7} &{#8} &{#9}
                     \end{smallmatrix}\right)}
                     
\newcommand{\linf}{l^{\infty}}		%l-infinity norm
\newcommand{\borel}{\operatorname{Borel}}	
\newcommand{\fa}{\forall}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\ip}[2]{\left\la #1,#2 \right\ra}
\renewcommand{\o}{\overline}
\renewcommand{\u}{\underline}
\newcommand{\h}{\hat}
\renewcommand{\r}{\rightarrow}
\newcommand{\xr}{\xrightarrow}
\newcommand{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\de}[2]{\frac{d #1}{d #2}}
\newcommand{\ddx}{\frac{d}{dx}}
\newcommand{\norm}[1]{\|#1\|} 
\newcommand{\tnorm}[1]{||#1||} % two-norm, i.e., with two bars
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\rw}{\rightharpoonup}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\pair}[1]{\left(#1\right)}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\wh}{\widehat}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\pv}{\operatorname{PV}}
\newcommand{\curl}{\operatorname{curl}}
\newcommand{\ds}{\displaystyle}
\newcommand{\inv}{^{-1}}
\newcommand{\dg}[1]{\textnormal{deg(#1)}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\ind}{\operatorname{Ind}}
\newcommand{\im}{\operatorname{im}}

%% In an integral, for the differential term
%\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\diff}{\, d}
%% For denoting powers of a differential term
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

%% integral with space removed
\newcommand{\myint}{\int\!}

\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceil }
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor }


%% PH stuff?
\newcommand{\pathhom}{\mathbf{PathHom}}
\newcommand{\dfchom}{\mathbf{DFCHom}}

\newcommand{\mlp}[1]{K^{\rightarrow}_{n_1,\ldots,n_{#1}}} 
\newcommand{\mlpgraph}[1]{K_{n_1,\ldots,n_{#1}}} 


\newcommand{\db}{d_{\operatorname{B}}}
\newcommand{\dgm}{\operatorname{Dgm}}
\newcommand{\vr}{\operatorname{VR}}
\newcommand{\cech}{\check{\operatorname{C}}}
\newcommand{\pvec}{{\operatorname{\mathbf{PVec}}}}
\newcommand{\pers}{{\operatorname{\mathbf{Pers}}}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\di}{d_{\operatorname{I}}}

\newcommand{\src}{\mf{D}^{\operatorname{so}}}
\newcommand{\sink}{\mf{D}^{\operatorname{si}}}

\newcommand{\so}{\operatorname{so}}
\newcommand{\si}{\operatorname{si}}



\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}


\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{defn}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem*{comments}{Comments}
%

\newenvironment{subproof}[1][\proofname]{%
  \renewcommand{\qedsymbol}{$\blacksquare$}%
  \begin{proof}[#1]%
}{%
  \end{proof}%
}

%% for align right within equation
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother



==> packages.tex <==


%\usepackage{arxiv}

\usepackage{booktabs} 
\usepackage{nicefrac}  
\usepackage{microtype}
\usepackage[utf8]{inputenc}

%\usepackage{enumitem}
%\usepackage{times}
%\usepackage{amsaddr}
%\usepackage[margin=1in]{geometry}

% \usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{multirow}

%\usepackage{url}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}
%\usepackage[normalem]{ulem}
%\usepackage{mathabx}
\usepackage{bbm}
\usepackage{array}
\usepackage[colorlinks=true,urlcolor=purple,
linkcolor=purple,citecolor=purple]{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{float}

% tables and figures
\usepackage{lscape}
\usepackage{graphicx}

% for nicer tables
\usepackage{booktabs}
\usepackage{longtable}
% \usepackage[skip=0pt, font=sc]{caption}
\usepackage{threeparttable}
\usepackage{threeparttablex}
% \usepackage[capposition=top]{floatrow}


\usepackage{mathrsfs}
%\usepackage{framed}
%\usepackage{latexsym}
%\usepackage{pb-diagram}
%\usepackage[mathscr]{}
\usepackage{graphicx}
%\usepackage[all]{xy} 
%\usepackage{color}
\usepackage{natbib}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{thmtools,thm-restate} %%for restating results 
%\usepackage[usenames, dvipsnames]{color}

\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\bfseries}}
\makeatother

%% TIK-Z RELATED PACKAGES
\usepackage{tikz}
\usetikzlibrary{decorations.markings, backgrounds, calc, positioning, shapes, shadows, arrows, fit, automata}
\usepackage{tikz-cd}
% Nice arrowheads
\usetikzlibrary{arrows.meta}
%\tikzset{>={Latex[length=3mm,width=2mm]}}
\tikzset{>={Latex}}



==> raw/table_tokens_spearmanr_weighted_no_field_df_title.tex <==
\begin{tabularx}{\textwidth}{XXXXXXXX}
\toprule
\multicolumn{4}{c}{Increasing utilization}&\multicolumn{4}{c}{ Decreasing utilization}\\
\cmidrule(lr){1-4}\cmidrule(lr){5-8}
\multicolumn{2}{c}{Papers}&\multicolumn{2}{c}{Patents}&\multicolumn{2}{c}{Papers}&\multicolumn{2}{c}{Patents}\\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Lemma&$r$&Lemma&$r$&Lemma&$r$&Lemma&$r$\\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}
\textcolor{c_color}{use}&0.9974&\textcolor{c_color}{base}&0.9983&\textcolor{d_color}{prove}&-0.2485&draw&-0.7409\\
\textcolor{d_color}{trigger}&0.9915&\textcolor{c_color}{use}&0.9983&\textcolor{d_color}{label}&-0.2510&\textcolor{c_color}{recover}&-0.7429\\
\textcolor{c_color}{assess}&0.9911&\textcolor{c_color}{provide}&0.9944&\textcolor{c_color}{illustrate}&-0.2615&foam&-0.7439\\
\textcolor{d_color}{generate}&0.9890&identify&0.9905&germinate&-0.2681&\textcolor{c_color}{copy}&-0.7473\\
predict&0.9880&\textcolor{c_color}{optimize}&0.9894&educate&-0.2703&dry&-0.7499\\
\textcolor{d_color}{link}&0.9866&\textcolor{d_color}{manufacture}&0.9871&drop&-0.2873&\textcolor{d_color}{substitute}&-0.7504\\
\textcolor{d_color}{define}&0.9856&determine&0.9843&\textcolor{d_color}{attack}&-0.2984&finish&-0.7510\\
\textcolor{c_color}{mediate}&0.9854&\textcolor{c_color}{store}&0.9843&\textcolor{c_color}{administer}&-0.3026&\textcolor{d_color}{lift}&-0.7513\\
interact&0.9853&\textcolor{c_color}{associate}&0.9829&\textcolor{c_color}{resemble}&-0.3384&\textcolor{c_color}{exercise}&-0.7529\\
\textcolor{c_color}{support}&0.9847&distribute&0.9826&judge&-0.3412&seal&-0.7625\\
\textcolor{c_color}{base}&0.9847&\textcolor{d_color}{create}&0.9824&\textcolor{d_color}{look}&-0.3417&\textcolor{d_color}{separate}&-0.7641\\
\textcolor{d_color}{detect}&0.9830&\textcolor{c_color}{perform}&0.9821&\textcolor{d_color}{dissect}&-0.3448&\textcolor{d_color}{propel}&-0.7644\\
dominate&0.9828&comprise&0.9815&\textcolor{d_color}{purify}&-0.3700&\textcolor{d_color}{prepare}&-0.7703\\
\textcolor{c_color}{optimize}&0.9818&\textcolor{c_color}{implement}&0.9804&\textcolor{c_color}{compose}&-0.3859&\textcolor{d_color}{spin}&-0.7709\\
\textcolor{d_color}{induce}&0.9810&\textcolor{d_color}{enable}&0.9793&\textcolor{c_color}{let}&-0.4289&\textcolor{d_color}{crack}&-0.7748\\
\textcolor{d_color}{drive}&0.9808&predict&0.9787&\textcolor{d_color}{bombard}&-0.4460&\textcolor{c_color}{stabilize}&-0.7790\\
identify&0.9807&access&0.9784&\textcolor{c_color}{disseminate}&-0.4590&lubricate&-0.7832\\
\textcolor{c_color}{model}&0.9794&\textcolor{d_color}{automate}&0.9779&\textcolor{c_color}{surface}&-0.4605&cut&-0.8064\\
\textcolor{c_color}{revisit}&0.9787&allocate&0.9776&\textcolor{c_color}{occur}&-0.4859&\textcolor{d_color}{melt}&-0.8118\\
assist&0.9782&\textcolor{c_color}{manage}&0.9770&\textcolor{d_color}{precipitate}&-0.5308&saw&-0.8143\\
\textcolor{c_color}{match}&0.9779&form&0.9768&\textcolor{c_color}{sing}&-0.6272&actuate&-0.8286\\
\textcolor{d_color}{incorporate}&0.9765&\textcolor{c_color}{record}&0.9765&\textcolor{d_color}{attempt}&-0.6634&\textcolor{d_color}{travel}&-0.8314\\
\textcolor{d_color}{target}&0.9750&\textcolor{c_color}{update}&0.9756&\textcolor{d_color}{produce}&-0.6754&\textcolor{d_color}{lay}&-0.8317\\
\textcolor{d_color}{construct}&0.9735&configure&0.9747&destroy&-0.6987&cast&-0.8378\\
\textcolor{c_color}{suppress}&0.9732&\textcolor{d_color}{integrate}&0.9737&\textcolor{d_color}{pour}&-0.7407&grind&-0.8401\\
distribute&0.9729&rout&0.9734&call&-0.7598&wind&-0.8513\\
\textcolor{d_color}{probe}&0.9729&\textcolor{d_color}{generate}&0.9723&\textcolor{d_color}{note}&-0.7769&strip&-0.8535\\
\textcolor{c_color}{enhance}&0.9723&\textcolor{d_color}{estimate}&0.9711&\textcolor{d_color}{encounter}&-0.8173&\textcolor{c_color}{indicate}&-0.8602\\
\textcolor{c_color}{update}&0.9721&\textcolor{c_color}{relate}&0.9706&excise&-0.8749&burn&-0.8742\\
\textcolor{c_color}{improve}&0.9719&\textcolor{c_color}{evaluate}&0.9703&concern&-0.9615&mean&-0.9672\\
\bottomrule
\end{tabularx}
